Alternative Input Signals Ease Transfer in Multilingual Machine Translation

Recent work in multilingual machine translation (MMT) has focused on the potential of positive transfer between languages, particularly cases where higher-resourced languages can benefit lower-resourced ones. While training an MMT model, the supervision signals learned from one language pair can be transferred to the other via the tokens shared by multiple source languages. However, the transfer is inhibited when the token overlap among source languages is small, which manifests naturally when languages use different writing systems. In this paper, we tackle inhibited transfer by augmenting the training data with alternative signals that unify different writing systems, such as phonetic, romanized, and transliterated input. We test these signals on Indic and Turkic languages, two language families where the writing systems differ but languages still share common features. Our results indicate that a straightforward multi-source self-ensemble -- training a model on a mixture of various signals and ensembling the outputs of the same model fed with different signals during inference, outperforms strong ensemble baselines by 1.3 BLEU points on both language families. Further, we find that incorporating alternative inputs via self-ensemble can be particularly effective when training set is small, leading to +5 BLEU when only 5% of the total training data is accessible. Finally, our analysis demonstrates that including alternative signals yields more consistency and translates named entities more accurately, which is crucial for increased factuality of automated systems.

==> other/links <==
- Indic results can be found in this spreadsheet: https://docs.google.com/spreadsheets/d/1EHtgZ9dz3-4hTAO7tJptJwIEwadqA9sz0j0vgOYsYlk/edit?usp=sharing
    
    - `exp-config' tab contains the configuration of each model, whose detailed results of each translation direction can be found under the `res' tab
    - `lc-res' contains the results of learning curve experiments
    - `ensemble-summary' contains the aggregated results of ensemble models (ensemble baseline, multi-source ensemble, multi-source self-ensemble)
    - `analysis' tab contains preliminary token-overlap stats 
    - `tables' contains the table1/2/3 in this paper
    - `speed-analysis' contains the sentence/sec of each translation direction while testing on my own devfair machine (not shared with others)
    - `enc-repr-analysis' contains the normalized euclidean distances among source language pairs (these results are included in the appendix as they are not conclusive enough)
    - `output-consistency' contains the results of C-BLEU for each source language pair and the aggregated results
    - `signal-example' figure4 in appendix
    - `signal-example-all' figure5 in appendix

- Turkic results can be found in this spreadsheet: https://docs.google.com/spreadsheets/d/13jdQQb-Kly7yxSHnFoFsyTf06X6xGcyTxb9EEXwBFbQ/edit?usp=sharing
    - tabs are most similar to the Indic sheet
    - `ky-romani' contains my manual alignment from ky alphabet to latin alphabet
    - `kk-romani' kk's cyrillic alphabet to latin
    - `az-cyrillic' az's original latin alphabet to cyrillic
    - `uz-cyrillic' uz's original latin alphabet to cyrillic

- figure_1 drawio file is added in the same folder, to open it go to \url{www.draw.io}

- backup: https://drive.google.com/drive/folders/1dXMxwmo3NNVL5-AeheCAkj94mEr2Ijza?usp=sharing




